Fair Notification Optimization: An Auction Approach

Notifications are important for the user experience in mobile apps and can influence their engagement. However, too many notifications can be disruptive for users. A typical mobile app usually has several types of notification, managed by distinct teams with objectives that are possibly conflicting with each other, or even with the overall platform objective. Therefore, there is a need for careful curation of notifications sent to users of these different types. In this work, we study a novel centralized approach for notification optimization, where we view the opportunities to send user notifications as items and types of notifications as buyers in an auction market. Furthermore, the auction setup is unique, and the platform has the ability to subsidize the bids from the notification types. Using tools from fair division, we study the application of competitive equilibrium for addressing this problem. We show that an Eisenberg-Gale-style convex program allows us to find an allocation that is fair to all notification types in hindsight. Using the dual of the formulation, we present an online algorithm that allocates notifications via first-price auctions using a pacing-multiplier approach. Secondly, we introduce an approach based on second-price auctions and pacing, which has the benefit of working well with existing advertising systems built for second-price auctions. Through an A/B test in production, we show that the second price-based auction system improves over a decentralized notification optimization system, leading to its launch in production for some Instagram notifications. Further, through simulations on Instagram notification data and a subsequent production A/B test, we compare the outcomes of first-price and second-price auctions and show that the former has more stable pacing multipliers.

==> item_arrive_online.tex <==
\subsection{Items arrive online, buyers and platform fixed}
Suppose that we know the set of buyers $i=1,\ldots, n$, but the items arrive sequentially, with one item arriving at every time step $t$, with valuation $v_{it}$ for each buyer $i$, platform valuations $v_{pit}$, and supply one.
In that case, the hindsight optimization problem that we would like to have solved after $T$ iterations is \cref{eq:mnw}, but where the indices $j$ correspond to the time steps, and $m=T$.
To handle the online arrival of items, we will extend the \emph{PACE} (Pace According to Current Estimated Utility) algorithm of \citet{gao2021online}. To that end, we will focus on the dual \cref{eq:mnw dual}, and we simplify \cref{eq:mnw dual} to get rid of the prices. This gives:
\begin{align}
\begin{array}{rlll}
    \min & \displaystyle \sum_j s_j \max_{i} (\beta_i v_{ij} + \beta_p v_{pij}) - \sum_{i\in T} B_i \log \beta_i - B_p\log\beta_p  \\
\end{array}    
\label{eq:mnw dual beta only}
\end{align}
For the purposes of this section, it will be convenient to assume that $\|B\|_1=1$, which can be achieved with rescaling and is without loss of generality. We also assume that there is some underlying distribution $\mu$ over a (possibly uncountable) space of items $\Theta$ such that $v_{it} = v_i(\theta_t)$, if item $\theta_t\in \Theta$ appears at time $t$. We assume that buyer valuations are normalized in the sense that for each $i\in \{1,\ldots,n\}$, $\mathbb E_{\theta} [v_i(\theta) ] =1$. For the platform we assume $u_p^* = 1$, where $u_p^*$ is the value achieved when solving the (possibly infinite-dimensional) allocation problem where the supply function $\mu$ is treated as supply, and the objective is the platform welfare. 

The PACE extension to the setting with a platform buyer works as follows. We learn a sequence pf pacing multipliers $\beta_i^t,\beta_p^t$. Then at each time $t$, the item is allocated via first-price auction, where each buyer bids $\beta_i^t v_{it} + \beta_p^t v_{pit}$, the item is allocated to the highest bidder, and they pay their bid. Then, the buyers and the platform update their pacing multipliers via a time-averaged estimate of $\beta^*$.
Formally, the steps at time $t$ are:
\begin{enumerate}
    \item Each buyer bids $\beta_i^t v_{it} + \beta_p^t v_{pit}$.
    \item The item is allocated to the highest bidder $i_t = \arg\max_{i\in [n]} \beta_i^t v_{it} + \beta_p^t v_{pit}$, with ties broken arbitrarily. The winner pays $\beta_{i_t}^t v_{{i_t}t} + \beta_p^t v_{pi_{t}t}$.
    \item Buyers recieve utilities $u_i^t = v_{it} \mathbb I\{i=i_t\}$, which is zero for all $i\ne i_t$. The platform receives $u_p^t = v_{pi_tt}$.
    \item Each buyer or platform $i\in \{1,\ldots,n,p\}$ updates their cumulative average utility  $\bar u_i^t = (1/t)\sum_{\tau=1}^t u_i^t$.
    \item New pacing multipliers are computed for each $i\in \{1,\ldots, n, p\}$:
    	\[
            \beta_i^{t+1} = \Pi_{l_i,h_i}(B_i / \bar u_i^t) = \min\left\{ \max\{l_i,B_i/\bar u_i^t\}, h_i \right\},
        \]
        where $l_i = B_i / (1+\delta_0)$ and $h_i = 1+\delta_0$ for some fixed $\delta_0 > 0$ (e.g. $\delta_0 = 0.05$).
\end{enumerate}

Note that the upper and lower bounds on $\beta$ require us to know the sum of valuations for each buyer, as well as $u_p^*$ (since we normalized valuations based on these quantities). If these are not known then lower bounds will suffice. For example, any constant factor bound will have no effect on the asymptotic convergence guarantee.
Using the same idea as in \citet{gao2020first}, we can now conclude strong convexity of the objective \cref{eq:mnw dual beta only} on the feasible set for $\beta$, because each $\beta$ is bounded above. A concern here could be that the upper bounds $h_i$ may cut off the optimal solution to \cref{eq:mnw dual beta only}, since we started out with no upper bound. However, based on the lower bounds on utility in \cref{claim:buyer proportionality,claim:platform proportionality}, and the fact that $\beta_i = B_i / u_i$ in equilibrium, we get that $\beta$ must strictly satisfy these upper bounds.

% One can similarly show that the lower bounds 

\begin{theorem}
    PACE generates pacing multipliers $\beta^t$ (where we include the platform multiplier $\beta_p^t$ in this vector) such that 
    \[
        \bbE \|\beta^t - \beta^*\|^2 \leq \frac{(6+\log t)G^2}{t\sigma^2},
    \]
    where $G^2 = \max_{i\in \{1,\ldots,n,p\}} \bbE_{\theta\sim \mu}[v_i(\theta)^2]$ and $\sigma = \frac{\min_{i\in \{1,\ldots,n,p\}}B_i}{(1+\delta_0)^2}$.
    \label{thm:items online pace}
\end{theorem}
\begin{proof}
    This follows by interpreting PACE as dual averaging (DA) in the composite setting without an auxiliary regularizer. 
    Consider the problem
    \[
        \min_w \E f_z(w) + \Psi(w),
    \]
    where $f_z(w)$ is a convex and subdifferentiably function for each point $z\in Z$ for some arbitrary sample space, and $\Psi$ is a strongly convex function. 
    At iteration $t$, let $f_t$ be the observed convex function, let $g^t\in \partial f_t(w^t)$, and then the \emph{dual average} is $\bar g^t = \sum_{\tau=1}^t \frac{1}{t} g^t$.
    DA without an auxiliary regularizer uses the update rule
    \[
        w^{t+1} = \arg\min_w \langle \bar g^t,w\rangle + \Psi(w).
    \]
    Going back to \cref{eq:mnw dual beta only}, we let $f_t = s_t\max_i (\beta_i v_{it} + \beta_p v_{pit})$ (as a function of $\beta$), and $\Psi = -\sum_i B_i\log \beta_i - B_p\log\beta_p$, with domain equal to $\beta_i \in [l_i,h_i]$ for each $i\in \{1,\ldots,n,p\}$. Now it is straightforward to see that $u_i^t$ is the subgradient $g^t$, $\bar u_i^t$ is the dual average, and the update rule for pacing multipliers is the DA rule.

    Now, invoking \citet[Theorem 2]{gao2021online}, which is itself a direct consequence of the proof of Corrolary 4 in \citet{xiao2010dual}, yields the bound.
\end{proof}

Moreover, by the bounds on performance of DA under nonstationary inputs developed by \citet{liao2022nonstationary}, we get that similar guarantees hold, up to a measure of nonstationarity, for ergodic, adversarially-corrupted, and periodic inputs.
\ck{Instantiate this, or not worth it?}




==> online_pairs.tex <==

\subsection{Pairs Arriving Online}

At each time step $t=1,\ldots, T$, a buyer valuation matrix $v^t \in \mathbb R^{n\times m}_+$ and a platform valuation matrix $v^t_p \in \mathbb R^{n\times m}_+$ is revealed. The goal is to compute a sequence of per-time-step allocations $x^1,\ldots, x^T$ such that each item satisfies its \emph{across timestep supply constraint} $\sum_{i=1}^n\sum_{t=1}^T x_{ij}^t \leq s_j$ for each item, and furthermore each item must satisfy its \emph{per-time-step supply constraint} $\sum_{i=1}^n x_{ij}^t \leq s_j^t$.

Now, since we want to perform the allocation online, it will be useful to reformulate this problem in order to get rid of the $\lambda_j^t$ variables. After reformulating we get the following dual problem (where $[\cdot ]^+$ denotes thresholding at zero)
\begin{align}
    \min_{p\geq 0,\beta \geq 0} 
    & \sum_{j=1}^m\sum_{t=1}^T s_j^t \left[ \max_{i} \left(\beta_i v_{ij}^t + \beta_p v_{pij}^t - p_j \right) \right]^+
    + \sum_{j=1}^m s_j p_j
    - \sum_{i=1}^n B_i \log \beta_i   
    - B_p \log \beta_p. 
    \label{eq:mnw pairs dual}
\end{align}


\subsection{Online Dual Averaging}

Consider the following algorithm for each time $t$:
\begin{itemize}
    \item An item $j$ is sampled, along with valuations $v_{ij}^t, v_{pij}^t$ (could be zero for some buyers)
    \item Each buyer submits a bid $\beta_i^t v_{ij}^t + \beta_p^t v_{pij}^t$
    \item If $\max_i \beta_i^t v_{ij}^t + \beta_p^t v_{pij}^t \geq p_j^t$, then let $i_t^*$ be the winner, and give them the item
    \item Let $x_{ij}^t = 0$ for all $i,j$ except $x_{i^*_tj}^t = 1$ if there is a winner
    \item Compute $\beta_i^{t+1}, \beta_p^{t+1}, p_j^{t+1}$ via online learning updates
\end{itemize}

Now let us consider a few options for online learning updates:

\paragraph{Basic online dual averaging}.
Let $u_i^t = v_{ij}^t x_{ij}^t$, $u_p^t = \sum_{i=1}^n v_{pij}^t x_{ij}^t$, and set 
\begin{align*}
\beta_i^{t+1} &= B_i / (\sum_{\tau = 1}^t u_i^\tau/t) \\
\beta_p^{t+1} &= B_p / (\sum_{\tau = 1}^t u_p^\tau/t) \\
p_j^{t+1} &= \eta_t ((s_j / T) - \sum_i x_{ij}^t) \\
\end{align*}
    
\subsubsection{Periodic Resolving}
Suppose that we set each user's price $p_j$ using some black box (for example, the price that would have yielded the right amount of notifications yesterday). 
We adopt such an approach, as oppose to online learning algorithms, because we need a price for each user, and we do not expect to see many auctions for an individual user (on the order of 10 per day is a realistic number). For that reason, we do not expect online learning methods to work well for setting prices.

Then, for a fixed set of prices $p$ for each user, we can use online learning to solve the following $\beta$ only dual:
\begin{align}
    \min_{\beta \geq 0} 
    & \sum_{j=1}^m\sum_{t=1}^T s_j^t \left[ \max_{i} \left(\beta_i v_{ij}^t + \beta_p v_{pij}^t - p_j \right) \right]^+
    - \sum_{i=1}^n B_i \log \beta_i   
    - B_p \log \beta_p. 
    \label{eq:mnw pairs dual beta only}
\end{align}


\textbf{The underlying solution}. 
Now suppose that we receive a set of predicted prices $p_j$ for each user $j$, and suppose that there is an underlying probability distribution $s\in L_+^\infty$ over possible valuation matrix pairs $\theta = (v, v_p)$. Suppose furthermore that the support of $s$ is contained in $[0,1]^{n\times m} \times [0,1]^{n\times m}$.

Suppose we treat each pair $\theta$ as an item with supply $s(\theta)$. In that case, we get an infinite-dimensional Fisher market whose market equilibria are described by the following convex program:
\begin{align}
    \min_{p\geq 0,\beta \geq 0} 
    & \sum_{j=1}^m \mathbb E_{(v_{ij},v_{pij}) \sim s} \left[ \max_{i} \left(\beta_i v_{ij} + \beta_p v_{pij} - p_j \right) \right]^+ \\&
    + \sum_{j=1}^m s_j p_j
    - \sum_{i=1}^n B_i \log \beta_i   
    - B_p \log \beta_p. 
    \label{eq:mnw pairs inf}
\end{align}
We call this the \emph{underlying market equilibrium}.
This is analogous to the infinite-dimensional Fisher market model of \citet{gao2022infinite}, except that we include the platform buyer $p$, and the per-user supplies $s_j$.
Their results about the relationship between solutions to \cref{eq:mnw pairs inf} and market equilibria easily extend to our setting, since the fact that valuations are contained in $[0,1]$ means that all measurability and integrability conditions are satisfied.
Thus, there is a vector $u^* \in \mathbb R_+^n$ describing the utilities achieved by each buyer $i$ in the underlying equilibrium; \citet{gao2022infinite} show that this utility vector satisfies the typical Fisher market guarantees such as Pareto optimality, envy-freeness, and proportionality.

\textbf{PACE algorithm}.
Now we show that if we are given the utility prices $p^* \in \mathbb R_+^m$ associated to the supply constraint for each user, then we can learn the pacing multipliers $\beta_i,\beta_p$ in an online fashion.
Our algorithm is an extension of the PACE (Pace According to Current Estimated utilities) algorithm of \citet{gao2021online}.

At each time $t$, PACE for our setting works as follows:
\begin{itemize}
    \item A valuation matrix pair $v^t,v_p^t$ is sampled from $s$
    \item Each buyer submits a bid $\beta_i^t v_{ij}^t + \beta_p^t v_{pij}^t$ for each user $j$
    \item For user $j$, if $\max_i \beta_i^t v_{ij}^t + \beta_p^t v_{pij}^t \geq p_j^*$, then let $i_t^*$ be the winner, and give them the item
    \item Let $x_{ij}^t = 0$ for all $i,j$ except $x_{i^*_tj}^t = 1$ if there is a winner
    \item Let $u_i^t = \sum_j v_{ij}^t x_{ij}^t, u_p^t = \sum_{ij} v_{pij}x_{ij}^t$
    \item Compute $\beta_i^{t+1}, \beta_p^{t+1}$ as follows
        \begin{align*}
        \beta_i^{t+1} &= B_i / (\sum_{\tau = 1}^t u_i^\tau/t) \\
        \beta_p^{t+1} &= B_p / (\sum_{\tau = 1}^t u_p^\tau/t)
        \end{align*}
\end{itemize}



\ck{Theorem about convergence}

\ck{show what happens when given arbitrary prices: guarantees for supplies that would have yielded those prices}

\ck{talk about different price options: solve hindsight EG, continuously update prices when exceeding supply, use most recent betas}

